Parameter Estimation for Low-Mass Eccentric Black Hole Binaries

Recent studies have shown that orbital eccentricity may indicate dynamical assembly as a formation mechanism for binary black holes. Eccentricity leaves a distinct signature in gravitational wave signals and it may be measured if the binary remains eccentric when it enters the LIGO band. Although eccentricity has not yet been confidently detected, the possibility of detecting eccentric binaries is becoming more likely with the improved sensitivity of gravitational wave detectors such as LIGO, Virgo, and KAGRA. It is crucial to assess the accuracy of current search pipelines in recovering eccentricity from gravitational wave signals if it is present. In this study, we investigate the ability of parameter estimation pipeline RIFT to recover eccentricity in the non-spinning and aligned-spin cases for low mass binary black holes. We use TaylorF2Ecc and TEOBResumS to inject sets of synthetic signals and test how well RIFT accurately recovers key binary black hole parameters. Our findings provide valuable insights into the capability of current parameter estimation methods to detect and measure eccentricity in gravitational wave signals.

==> Makefile <==
DOCS = paper.pdf

paper_FIGS = corner_mc_q_eccentricity.png output_pp_ecc_diag.pdf output_pp_f2_nondiag.pdf

paper_TABS =

paper_DEPS = biblio.bib \
                   $(notes_TABS) $(notes_FIGS)

BYPROD = paper.bbl paper.blg paper.ps \
         $(PDFFIGS) $(TEXFIGS)

default: $(DOCS) #gitID

#.PHONY: gitID
#gitID:
#	./git-tag.sh

paper.pdf: paper.tex $(paper_DEPS)
	latexmk -pdf paper.tex

paper.bbl: paper.pdf

%.pdf: %.tex
	pdflatex $< && pdflatex $<

%.pdf: %.eps
	epstopdf --outfile=$@ $(@:.pdf=.eps)

%.md: %.tex
	pandoc -t markdown $(@:.md=.tex) > $@

clean:
	rm -f *.aux *.log *.out *.dvi $(DOCS) $(BYPROD)

